First Measurement of the $D_s^+\rightarrow K^0\mu^+\nu_{\mu}$ Decay

We report the first measurement of the semileptonic decay $D^+_s \rightarrow K^0\mu^+\nu_{\mu}$, using a sample of $e^+e^-$ annihilation data corresponding to an integrated luminosity of $7.33~\mathrm{fb}^{-1}$ collected at center-of-mass energies between 4.128 to 4.226~GeV with the BESIII detector at the BEPCII collider. The branching fraction of the decay is measured to be $\mathcal{B}(D^+_s\rightarrow K^0\mu^+\nu_{\mu}) = (2.89 \pm 0.27_{\rm stat} \pm 0.12_{\rm syst})\times 10^{-3}$, where the first uncertainty is statistical and the second is systematic. Based on a simultaneous fit to the partial decay rates in $q^2$ intervals measured in $D^+_s \rightarrow K^0\mu^+\nu_{\mu}$ and $D^+_s \rightarrow K^0e^+\nu_{e}$ decays, the product value of the form factor $f^{K^0}_{+}(0)$ and the Cabibbo-Kobayashi-Maskawa matrix element $|V_{cd}|$ is measured to be $f^{K^0}_{+}(0)|V_{cd}|=0.140\pm0.008_{\rm stat}\pm0.002_{\rm syst}$. Using $|V_{cd}|=0.22486\pm0.00068$ as an input, the hadronic form factor is determined to be $f^{K^0}_{+}(0)=0.623\pm0.036_{\rm stat} \pm 0.009_{\rm syst}$ at $q^2=0$. This is the most precise determination of $f^{K^0}_{+}(0)$ in the $D^+_s \rightarrow K^0$ transition to date. The measured branching fraction and form factor presented in this work provide the most stringent test on various non-perturbative theoretical calculations. Taking $f^{K^0}_{+}(0)=0.6307\pm0.0020$ from lattice calculations as an input, we obtain $|V_{cd}|=0.220\pm0.013_{\rm stat}\pm0.003_{\rm syst}\pm0.001_{\rm LQCD}$, which is the most precise determination of $|V_{cd}|$ using the $D_s^+\rightarrow K^0\ell^+\nu_{\ell}$ decays. In addition, lepton flavor universality is tested for the first time with $D^+_s \rightarrow K^0\ell^+\nu_{\ell}$ decays in full and separate $q^2$ intervals. No obvious violation is found.

==> authorlist_2025-04-17.tex <==
%% Saved at => 2025-04-17
M.~Ablikim$^{1}$, M.~N.~Achasov$^{4,d}$, P.~Adlarson$^{77}$, X.~C.~Ai$^{82}$, R.~Aliberti$^{36}$, A.~Amoroso$^{76A,76C}$, Q.~An$^{73,59,b}$, Y.~Bai$^{58}$, O.~Bakina$^{37}$, Y.~Ban$^{47,i}$, H.-R.~Bao$^{65}$, V.~Batozskaya$^{1,45}$, K.~Begzsuren$^{33}$, N.~Berger$^{36}$, M.~Berlowski$^{45}$, M.~Bertani$^{29A}$, D.~Bettoni$^{30A}$, F.~Bianchi$^{76A,76C}$, E.~Bianco$^{76A,76C}$, A.~Bortone$^{76A,76C}$, I.~Boyko$^{37}$, R.~A.~Briere$^{5}$, A.~Brueggemann$^{70}$, H.~Cai$^{78}$, M.~H.~Cai$^{39,l,m}$, X.~Cai$^{1,59}$, A.~Calcaterra$^{29A}$, G.~F.~Cao$^{1,65}$, N.~Cao$^{1,65}$, S.~A.~Cetin$^{63A}$, X.~Y.~Chai$^{47,i}$, J.~F.~Chang$^{1,59}$, G.~R.~Che$^{44}$, Y.~Z.~Che$^{1,59,65}$, C.~H.~Chen$^{9}$, Chao~Chen$^{56}$, G.~Chen$^{1}$, H.~S.~Chen$^{1,65}$, H.~Y.~Chen$^{21}$, M.~L.~Chen$^{1,59,65}$, S.~J.~Chen$^{43}$, S.~L.~Chen$^{46}$, S.~M.~Chen$^{62}$, T.~Chen$^{1,65}$, X.~R.~Chen$^{32,65}$, X.~T.~Chen$^{1,65}$, X.~Y.~Chen$^{12,h}$, Y.~B.~Chen$^{1,59}$, Y.~Q.~Chen$^{35}$, Y.~Q.~Chen$^{16}$, Z.~Chen$^{25}$, Z.~J.~Chen$^{26,j}$, Z.~K.~Chen$^{60}$, S.~K.~Choi$^{10}$, X. ~Chu$^{12,h}$, G.~Cibinetto$^{30A}$, F.~Cossio$^{76C}$, J.~Cottee-Meldrum$^{64}$, J.~J.~Cui$^{51}$, H.~L.~Dai$^{1,59}$, J.~P.~Dai$^{80}$, A.~Dbeyssi$^{19}$, R.~ E.~de Boer$^{3}$, D.~Dedovich$^{37}$, C.~Q.~Deng$^{74}$, Z.~Y.~Deng$^{1}$, A.~Denig$^{36}$, I.~Denysenko$^{37}$, M.~Destefanis$^{76A,76C}$, F.~De~Mori$^{76A,76C}$, B.~Ding$^{68,1}$, X.~X.~Ding$^{47,i}$, Y.~Ding$^{41}$, Y.~Ding$^{35}$, Y.~X.~Ding$^{31}$, J.~Dong$^{1,59}$, L.~Y.~Dong$^{1,65}$, M.~Y.~Dong$^{1,59,65}$, X.~Dong$^{78}$, M.~C.~Du$^{1}$, S.~X.~Du$^{82}$, S.~X.~Du$^{12,h}$, Y.~Y.~Duan$^{56}$, P.~Egorov$^{37,c}$, G.~F.~Fan$^{43}$, J.~J.~Fan$^{20}$, Y.~H.~Fan$^{46}$, J.~Fang$^{1,59}$, J.~Fang$^{60}$, S.~S.~Fang$^{1,65}$, W.~X.~Fang$^{1}$, Y.~Q.~Fang$^{1,59}$, R.~Farinelli$^{30A}$, L.~Fava$^{76B,76C}$, F.~Feldbauer$^{3}$, G.~Felici$^{29A}$, C.~Q.~Feng$^{73,59}$, J.~H.~Feng$^{16}$, L.~Feng$^{39,l,m}$, Q.~X.~Feng$^{39,l,m}$, Y.~T.~Feng$^{73,59}$, M.~Fritsch$^{3}$, C.~D.~Fu$^{1}$, J.~L.~Fu$^{65}$, Y.~W.~Fu$^{1,65}$, H.~Gao$^{65}$, X.~B.~Gao$^{42}$, Y.~Gao$^{73,59}$, Y.~N.~Gao$^{20}$, Y.~N.~Gao$^{47,i}$, Y.~Y.~Gao$^{31}$, S.~Garbolino$^{76C}$, I.~Garzia$^{30A,30B}$, L.~Ge$^{58}$, P.~T.~Ge$^{20}$, Z.~W.~Ge$^{43}$, C.~Geng$^{60}$, E.~M.~Gersabeck$^{69}$, A.~Gilman$^{71}$, K.~Goetzen$^{13}$, J.~D.~Gong$^{35}$, L.~Gong$^{41}$, W.~X.~Gong$^{1,59}$, W.~Gradl$^{36}$, S.~Gramigna$^{30A,30B}$, M.~Greco$^{76A,76C}$, M.~H.~Gu$^{1,59}$, Y.~T.~Gu$^{15}$, C.~Y.~Guan$^{1,65}$, A.~Q.~Guo$^{32}$, L.~B.~Guo$^{42}$, M.~J.~Guo$^{51}$, R.~P.~Guo$^{50}$, Y.~P.~Guo$^{12,h}$, A.~Guskov$^{37,c}$, J.~Gutierrez$^{28}$, K.~L.~Han$^{65}$, T.~T.~Han$^{1}$, F.~Hanisch$^{3}$, K.~D.~Hao$^{73,59}$, X.~Q.~Hao$^{20}$, F.~A.~Harris$^{67}$, K.~K.~He$^{56}$, K.~L.~He$^{1,65}$, F.~H.~Heinsius$^{3}$, C.~H.~Heinz$^{36}$, Y.~K.~Heng$^{1,59,65}$, C.~Herold$^{61}$, P.~C.~Hong$^{35}$, G.~Y.~Hou$^{1,65}$, X.~T.~Hou$^{1,65}$, Y.~R.~Hou$^{65}$, Z.~L.~Hou$^{1}$, H.~M.~Hu$^{1,65}$, J.~F.~Hu$^{57,k}$, Q.~P.~Hu$^{73,59}$, S.~L.~Hu$^{12,h}$, T.~Hu$^{1,59,65}$, Y.~Hu$^{1}$, Z.~M.~Hu$^{60}$, G.~S.~Huang$^{73,59}$, K.~X.~Huang$^{60}$, L.~Q.~Huang$^{32,65}$, P.~Huang$^{43}$, X.~T.~Huang$^{51}$, Y.~P.~Huang$^{1}$, Y.~S.~Huang$^{60}$, T.~Hussain$^{75}$, N.~H\"usken$^{36}$, N.~in der Wiesche$^{70}$, J.~Jackson$^{28}$, Q.~Ji$^{1}$, Q.~P.~Ji$^{20}$, W.~Ji$^{1,65}$, X.~B.~Ji$^{1,65}$, X.~L.~Ji$^{1,59}$, Y.~Y.~Ji$^{51}$, Z.~K.~Jia$^{73,59}$, D.~Jiang$^{1,65}$, H.~B.~Jiang$^{78}$, P.~C.~Jiang$^{47,i}$, S.~J.~Jiang$^{9}$, T.~J.~Jiang$^{17}$, X.~S.~Jiang$^{1,59,65}$, Y.~Jiang$^{65}$, J.~B.~Jiao$^{51}$, J.~K.~Jiao$^{35}$, Z.~Jiao$^{24}$, S.~Jin$^{43}$, Y.~Jin$^{68}$, M.~Q.~Jing$^{1,65}$, X.~M.~Jing$^{65}$, T.~Johansson$^{77}$, S.~Kabana$^{34}$, N.~Kalantar-Nayestanaki$^{66}$, X.~L.~Kang$^{9}$, X.~S.~Kang$^{41}$, M.~Kavatsyuk$^{66}$, B.~C.~Ke$^{82}$, V.~Khachatryan$^{28}$, A.~Khoukaz$^{70}$, R.~Kiuchi$^{1}$, O.~B.~Kolcu$^{63A}$, B.~Kopf$^{3}$, M.~Kuessner$^{3}$, X.~Kui$^{1,65}$, N.~~Kumar$^{27}$, A.~Kupsc$^{45,77}$, W.~K\"uhn$^{38}$, Q.~Lan$^{74}$, W.~N.~Lan$^{20}$, T.~T.~Lei$^{73,59}$, M.~Lellmann$^{36}$, T.~Lenz$^{36}$, C.~Li$^{48}$, C.~Li$^{44}$, C.~H.~Li$^{40}$, C.~K.~Li$^{21}$, D.~M.~Li$^{82}$, F.~Li$^{1,59}$, G.~Li$^{1}$, H.~B.~Li$^{1,65}$, H.~J.~Li$^{20}$, H.~N.~Li$^{57,k}$, Hui~Li$^{44}$, J.~R.~Li$^{62}$, J.~S.~Li$^{60}$, K.~Li$^{1}$, K.~L.~Li$^{39,l,m}$, K.~L.~Li$^{20}$, L.~J.~Li$^{1,65}$, Lei~Li$^{49}$, M.~H.~Li$^{44}$, M.~R.~Li$^{1,65}$, P.~L.~Li$^{65}$, P.~R.~Li$^{39,l,m}$, Q.~M.~Li$^{1,65}$, Q.~X.~Li$^{51}$, R.~Li$^{18,32}$, S.~X.~Li$^{12}$, T. ~Li$^{51}$, T.~Y.~Li$^{44}$, W.~D.~Li$^{1,65}$, W.~G.~Li$^{1,b}$, X.~Li$^{1,65}$, X.~H.~Li$^{73,59}$, X.~L.~Li$^{51}$, X.~Y.~Li$^{1,8}$, X.~Z.~Li$^{60}$, Y.~Li$^{20}$, Y.~G.~Li$^{47,i}$, Y.~P.~Li$^{35}$, Z.~J.~Li$^{60}$, Z.~Y.~Li$^{80}$, H.~Liang$^{73,59}$, Y.~F.~Liang$^{55}$, Y.~T.~Liang$^{32,65}$, G.~R.~Liao$^{14}$, L.~B.~Liao$^{60}$, M.~H.~Liao$^{60}$, Y.~P.~Liao$^{1,65}$, J.~Libby$^{27}$, A. ~Limphirat$^{61}$, C.~C.~Lin$^{56}$, D.~X.~Lin$^{32,65}$, L.~Q.~Lin$^{40}$, T.~Lin$^{1}$, B.~J.~Liu$^{1}$, B.~X.~Liu$^{78}$, C.~Liu$^{35}$, C.~X.~Liu$^{1}$, F.~Liu$^{1}$, F.~H.~Liu$^{54}$, Feng~Liu$^{6}$, G.~M.~Liu$^{57,k}$, H.~Liu$^{39,l,m}$, H.~B.~Liu$^{15}$, H.~H.~Liu$^{1}$, H.~M.~Liu$^{1,65}$, Huihui~Liu$^{22}$, J.~B.~Liu$^{73,59}$, J.~J.~Liu$^{21}$, K.~Liu$^{39,l,m}$, K. ~Liu$^{74}$, K.~Y.~Liu$^{41}$, Ke~Liu$^{23}$, L.~C.~Liu$^{44}$, Lu~Liu$^{44}$, M.~H.~Liu$^{12,h}$, P.~L.~Liu$^{1}$, Q.~Liu$^{65}$, S.~B.~Liu$^{73,59}$, T.~Liu$^{12,h}$, W.~K.~Liu$^{44}$, W.~M.~Liu$^{73,59}$, W.~T.~Liu$^{40}$, X.~Liu$^{39,l,m}$, X.~Liu$^{40}$, X.~K.~Liu$^{39,l,m}$, X.~L.~Liu$^{12,h}$, X.~Y.~Liu$^{78}$, Y.~Liu$^{39,l,m}$, Y.~Liu$^{82}$, Y.~Liu$^{82}$, Y.~B.~Liu$^{44}$, Z.~A.~Liu$^{1,59,65}$, Z.~D.~Liu$^{9}$, Z.~Q.~Liu$^{51}$, X.~C.~Lou$^{1,59,65}$, F.~X.~Lu$^{60}$, H.~J.~Lu$^{24}$, J.~G.~Lu$^{1,59}$, X.~L.~Lu$^{16}$, Y.~Lu$^{7}$, Y.~H.~Lu$^{1,65}$, Y.~P.~Lu$^{1,59}$, Z.~H.~Lu$^{1,65}$, C.~L.~Luo$^{42}$, J.~R.~Luo$^{60}$, J.~S.~Luo$^{1,65}$, M.~X.~Luo$^{81}$, T.~Luo$^{12,h}$, X.~L.~Luo$^{1,59}$, Z.~Y.~Lv$^{23}$, X.~R.~Lyu$^{65,q}$, Y.~F.~Lyu$^{44}$, Y.~H.~Lyu$^{82}$, F.~C.~Ma$^{41}$, H.~L.~Ma$^{1}$, J.~L.~Ma$^{1,65}$, L.~L.~Ma$^{51}$, L.~R.~Ma$^{68}$, Q.~M.~Ma$^{1}$, R.~Q.~Ma$^{1,65}$, R.~Y.~Ma$^{20}$, T.~Ma$^{73,59}$, X.~T.~Ma$^{1,65}$, X.~Y.~Ma$^{1,59}$, Y.~M.~Ma$^{32}$, F.~E.~Maas$^{19}$, I.~MacKay$^{71}$, M.~Maggiora$^{76A,76C}$, S.~Malde$^{71}$, Q.~A.~Malik$^{75}$, H.~X.~Mao$^{39,l,m}$, Y.~J.~Mao$^{47,i}$, Z.~P.~Mao$^{1}$, S.~Marcello$^{76A,76C}$, A.~Marshall$^{64}$, F.~M.~Melendi$^{30A,30B}$, Y.~H.~Meng$^{65}$, Z.~X.~Meng$^{68}$, G.~Mezzadri$^{30A}$, H.~Miao$^{1,65}$, T.~J.~Min$^{43}$, R.~E.~Mitchell$^{28}$, X.~H.~Mo$^{1,59,65}$, B.~Moses$^{28}$, N.~Yu.~Muchnoi$^{4,d}$, J.~Muskalla$^{36}$, Y.~Nefedov$^{37}$, F.~Nerling$^{19,f}$, L.~S.~Nie$^{21}$, I.~B.~Nikolaev$^{4,d}$, Z.~Ning$^{1,59}$, S.~Nisar$^{11,n}$, Q.~L.~Niu$^{39,l,m}$, W.~D.~Niu$^{12,h}$, C.~Normand$^{64}$, S.~L.~Olsen$^{10,65}$, Q.~Ouyang$^{1,59,65}$, S.~Pacetti$^{29B,29C}$, X.~Pan$^{56}$, Y.~Pan$^{58}$, A.~Pathak$^{10}$, Y.~P.~Pei$^{73,59}$, M.~Pelizaeus$^{3}$, H.~P.~Peng$^{73,59}$, X.~J.~Peng$^{39,l,m}$, Y.~Y.~Peng$^{39,l,m}$, K.~Peters$^{13,f}$, K.~Petridis$^{64}$, J.~L.~Ping$^{42}$, R.~G.~Ping$^{1,65}$, S.~Plura$^{36}$, V.~~Prasad$^{35}$, F.~Z.~Qi$^{1}$, H.~R.~Qi$^{62}$, M.~Qi$^{43}$, S.~Qian$^{1,59}$, W.~B.~Qian$^{65}$, C.~F.~Qiao$^{65}$, J.~H.~Qiao$^{20}$, J.~J.~Qin$^{74}$, J.~L.~Qin$^{56}$, L.~Q.~Qin$^{14}$, L.~Y.~Qin$^{73,59}$, P.~B.~Qin$^{74}$, X.~P.~Qin$^{12,h}$, X.~S.~Qin$^{51}$, Z.~H.~Qin$^{1,59}$, J.~F.~Qiu$^{1}$, Z.~H.~Qu$^{74}$, J.~Rademacker$^{64}$, C.~F.~Redmer$^{36}$, A.~Rivetti$^{76C}$, M.~Rolo$^{76C}$, G.~Rong$^{1,65}$, S.~S.~Rong$^{1,65}$, F.~Rosini$^{29B,29C}$, Ch.~Rosner$^{19}$, M.~Q.~Ruan$^{1,59}$, N.~Salone$^{45}$, A.~Sarantsev$^{37,e}$, Y.~Schelhaas$^{36}$, K.~Schoenning$^{77}$, M.~Scodeggio$^{30A}$, K.~Y.~Shan$^{12,h}$, W.~Shan$^{25}$, X.~Y.~Shan$^{73,59}$, Z.~J.~Shang$^{39,l,m}$, J.~F.~Shangguan$^{17}$, L.~G.~Shao$^{1,65}$, M.~Shao$^{73,59}$, C.~P.~Shen$^{12,h}$, H.~F.~Shen$^{1,8}$, W.~H.~Shen$^{65}$, X.~Y.~Shen$^{1,65}$, B.~A.~Shi$^{65}$, H.~Shi$^{73,59}$, J.~L.~Shi$^{12,h}$, J.~Y.~Shi$^{1}$, S.~Y.~Shi$^{74}$, X.~Shi$^{1,59}$, H.~L.~Song$^{73,59}$, J.~J.~Song$^{20}$, T.~Z.~Song$^{60}$, W.~M.~Song$^{35}$, Y. ~J.~Song$^{12,h}$, Y.~X.~Song$^{47,i,o}$, S.~Sosio$^{76A,76C}$, S.~Spataro$^{76A,76C}$, S~Stansilaus$^{71}$, F.~Stieler$^{36}$, S.~S~Su$^{41}$, Y.~J.~Su$^{65}$, G.~B.~Sun$^{78}$, G.~X.~Sun$^{1}$, H.~Sun$^{65}$, H.~K.~Sun$^{1}$, J.~F.~Sun$^{20}$, K.~Sun$^{62}$, L.~Sun$^{78}$, S.~S.~Sun$^{1,65}$, T.~Sun$^{52,g}$, Y.~C.~Sun$^{78}$, Y.~H.~Sun$^{31}$, Y.~J.~Sun$^{73,59}$, Y.~Z.~Sun$^{1}$, Z.~Q.~Sun$^{1,65}$, Z.~T.~Sun$^{51}$, C.~J.~Tang$^{55}$, G.~Y.~Tang$^{1}$, J.~Tang$^{60}$, J.~J.~Tang$^{73,59}$, L.~F.~Tang$^{40}$, Y.~A.~Tang$^{78}$, L.~Y.~Tao$^{74}$, M.~Tat$^{71}$, J.~X.~Teng$^{73,59}$, J.~Y.~Tian$^{73,59}$, W.~H.~Tian$^{60}$, Y.~Tian$^{32}$, Z.~F.~Tian$^{78}$, I.~Uman$^{63B}$, B.~Wang$^{60}$, B.~Wang$^{1}$, Bo~Wang$^{73,59}$, C.~Wang$^{39,l,m}$, C.~~Wang$^{20}$, Cong~Wang$^{23}$, D.~Y.~Wang$^{47,i}$, H.~J.~Wang$^{39,l,m}$, J.~J.~Wang$^{78}$, K.~Wang$^{1,59}$, L.~L.~Wang$^{1}$, L.~W.~Wang$^{35}$, M. ~Wang$^{73,59}$, M.~Wang$^{51}$, N.~Y.~Wang$^{65}$, S.~Wang$^{12,h}$, T. ~Wang$^{12,h}$, T.~J.~Wang$^{44}$, W.~Wang$^{60}$, W. ~Wang$^{74}$, W.~P.~Wang$^{36,59,73,p}$, X.~Wang$^{47,i}$, X.~F.~Wang$^{39,l,m}$, X.~J.~Wang$^{40}$, X.~L.~Wang$^{12,h}$, X.~N.~Wang$^{1,65}$, Y.~Wang$^{62}$, Y.~D.~Wang$^{46}$, Y.~F.~Wang$^{1,8,65}$, Y.~H.~Wang$^{39,l,m}$, Y.~J.~Wang$^{73,59}$, Y.~L.~Wang$^{20}$, Y.~N.~Wang$^{78}$, Y.~Q.~Wang$^{1}$, Yaqian~Wang$^{18}$, Yi~Wang$^{62}$, Yuan~Wang$^{18,32}$, Z.~Wang$^{1,59}$, Z.~L. ~Wang$^{74}$, Z.~L.~Wang$^{2}$, Z.~Q.~Wang$^{12,h}$, Z.~Y.~Wang$^{1,65}$, D.~H.~Wei$^{14}$, H.~R.~Wei$^{44}$, F.~Weidner$^{70}$, S.~P.~Wen$^{1}$, Y.~R.~Wen$^{40}$, U.~Wiedner$^{3}$, G.~Wilkinson$^{71}$, M.~Wolke$^{77}$, C.~Wu$^{40}$, J.~F.~Wu$^{1,8}$, L.~H.~Wu$^{1}$, L.~J.~Wu$^{20}$, L.~J.~Wu$^{1,65}$, Lianjie~Wu$^{20}$, S.~G.~Wu$^{1,65}$, S.~M.~Wu$^{65}$, X.~Wu$^{12,h}$, X.~H.~Wu$^{35}$, Y.~J.~Wu$^{32}$, Z.~Wu$^{1,59}$, L.~Xia$^{73,59}$, X.~M.~Xian$^{40}$, B.~H.~Xiang$^{1,65}$, D.~Xiao$^{39,l,m}$, G.~Y.~Xiao$^{43}$, H.~Xiao$^{74}$, Y. ~L.~Xiao$^{12,h}$, Z.~J.~Xiao$^{42}$, C.~Xie$^{43}$, K.~J.~Xie$^{1,65}$, X.~H.~Xie$^{47,i}$, Y.~Xie$^{51}$, Y.~G.~Xie$^{1,59}$, Y.~H.~Xie$^{6}$, Z.~P.~Xie$^{73,59}$, T.~Y.~Xing$^{1,65}$, C.~F.~Xu$^{1,65}$, C.~J.~Xu$^{60}$, G.~F.~Xu$^{1}$, H.~Y.~Xu$^{2}$, H.~Y.~Xu$^{68,2}$, M.~Xu$^{73,59}$, Q.~J.~Xu$^{17}$, Q.~N.~Xu$^{31}$, T.~D.~Xu$^{74}$, W.~Xu$^{1}$, W.~L.~Xu$^{68}$, X.~P.~Xu$^{56}$, Y.~Xu$^{41}$, Y.~Xu$^{12,h}$, Y.~C.~Xu$^{79}$, Z.~S.~Xu$^{65}$, F.~Yan$^{12,h}$, H.~Y.~Yan$^{40}$, L.~Yan$^{12,h}$, W.~B.~Yan$^{73,59}$, W.~C.~Yan$^{82}$, W.~H.~Yan$^{6}$, W.~P.~Yan$^{20}$, X.~Q.~Yan$^{1,65}$, H.~J.~Yang$^{52,g}$, H.~L.~Yang$^{35}$, H.~X.~Yang$^{1}$, J.~H.~Yang$^{43}$, R.~J.~Yang$^{20}$, T.~Yang$^{1}$, Y.~Yang$^{12,h}$, Y.~F.~Yang$^{44}$, Y.~H.~Yang$^{43}$, Y.~Q.~Yang$^{9}$, Y.~X.~Yang$^{1,65}$, Y.~Z.~Yang$^{20}$, M.~Ye$^{1,59}$, M.~H.~Ye$^{8,b}$, Z.~J.~Ye$^{57,k}$, Junhao~Yin$^{44}$, Z.~Y.~You$^{60}$, B.~X.~Yu$^{1,59,65}$, C.~X.~Yu$^{44}$, G.~Yu$^{13}$, J.~S.~Yu$^{26,j}$, L.~Q.~Yu$^{12,h}$, M.~C.~Yu$^{41}$, T.~Yu$^{74}$, X.~D.~Yu$^{47,i}$, Y.~C.~Yu$^{82}$, C.~Z.~Yuan$^{1,65}$, H.~Yuan$^{1,65}$, J.~Yuan$^{46}$, J.~Yuan$^{35}$, L.~Yuan$^{2}$, S.~C.~Yuan$^{1,65}$, X.~Q.~Yuan$^{1}$, Y.~Yuan$^{1,65}$, Z.~Y.~Yuan$^{60}$, C.~X.~Yue$^{40}$, Ying~Yue$^{20}$, A.~A.~Zafar$^{75}$, S.~H.~Zeng$^{64A,64B,64C,64D}$, X.~Zeng$^{12,h}$, Y.~Zeng$^{26,j}$, Y.~J.~Zeng$^{60}$, Y.~J.~Zeng$^{1,65}$, X.~Y.~Zhai$^{35}$, Y.~H.~Zhan$^{60}$, ~Zhang$^{71}$, A.~Q.~Zhang$^{1,65}$, B.~L.~Zhang$^{1,65}$, B.~X.~Zhang$^{1}$, D.~H.~Zhang$^{44}$, G.~Y.~Zhang$^{20}$, G.~Y.~Zhang$^{1,65}$, H.~Zhang$^{73,59}$, H.~Zhang$^{82}$, H.~C.~Zhang$^{1,59,65}$, H.~H.~Zhang$^{60}$, H.~Q.~Zhang$^{1,59,65}$, H.~R.~Zhang$^{73,59}$, H.~Y.~Zhang$^{1,59}$, J.~Zhang$^{60}$, J.~Zhang$^{82}$, J.~J.~Zhang$^{53}$, J.~L.~Zhang$^{21}$, J.~Q.~Zhang$^{42}$, J.~S.~Zhang$^{12,h}$, J.~W.~Zhang$^{1,59,65}$, J.~X.~Zhang$^{39,l,m}$, J.~Y.~Zhang$^{1}$, J.~Z.~Zhang$^{1,65}$, Jianyu~Zhang$^{65}$, L.~M.~Zhang$^{62}$, Lei~Zhang$^{43}$, N.~Zhang$^{82}$, P.~Zhang$^{1,8}$, Q.~Zhang$^{20}$, Q.~Y.~Zhang$^{35}$, R.~Y.~Zhang$^{39,l,m}$, S.~H.~Zhang$^{1,65}$, Shulei~Zhang$^{26,j}$, X.~M.~Zhang$^{1}$, X.~Y~Zhang$^{41}$, X.~Y.~Zhang$^{51}$, Y. ~Zhang$^{74}$, Y.~Zhang$^{1}$, Y. ~T.~Zhang$^{82}$, Y.~H.~Zhang$^{1,59}$, Y.~M.~Zhang$^{40}$, Y.~P.~Zhang$^{73,59}$, Z.~D.~Zhang$^{1}$, Z.~H.~Zhang$^{1}$, Z.~L.~Zhang$^{35}$, Z.~L.~Zhang$^{56}$, Z.~X.~Zhang$^{20}$, Z.~Y.~Zhang$^{44}$, Z.~Y.~Zhang$^{78}$, Z.~Z. ~Zhang$^{46}$, Zh.~Zh.~Zhang$^{20}$, G.~Zhao$^{1}$, J.~Y.~Zhao$^{1,65}$, J.~Z.~Zhao$^{1,59}$, L.~Zhao$^{73,59}$, L.~Zhao$^{1}$, M.~G.~Zhao$^{44}$, N.~Zhao$^{80}$, R.~P.~Zhao$^{65}$, S.~J.~Zhao$^{82}$, Y.~B.~Zhao$^{1,59}$, Y.~L.~Zhao$^{56}$, Y.~X.~Zhao$^{32,65}$, Z.~G.~Zhao$^{73,59}$, A.~Zhemchugov$^{37,c}$, B.~Zheng$^{74}$, B.~M.~Zheng$^{35}$, J.~P.~Zheng$^{1,59}$, W.~J.~Zheng$^{1,65}$, X.~R.~Zheng$^{20}$, Y.~H.~Zheng$^{65,q}$, B.~Zhong$^{42}$, C.~Zhong$^{20}$, H.~Zhou$^{36,51,p}$, J.~Q.~Zhou$^{35}$, J.~Y.~Zhou$^{35}$, S. ~Zhou$^{6}$, X.~Zhou$^{78}$, X.~K.~Zhou$^{6}$, X.~R.~Zhou$^{73,59}$, X.~Y.~Zhou$^{40}$, Y.~X.~Zhou$^{79}$, Y.~Z.~Zhou$^{12,h}$, A.~N.~Zhu$^{65}$, J.~Zhu$^{44}$, K.~Zhu$^{1}$, K.~J.~Zhu$^{1,59,65}$, K.~S.~Zhu$^{12,h}$, L.~Zhu$^{35}$, L.~X.~Zhu$^{65}$, S.~H.~Zhu$^{72}$, T.~J.~Zhu$^{12,h}$, W.~D.~Zhu$^{12,h}$, W.~D.~Zhu$^{42}$, W.~J.~Zhu$^{1}$, W.~Z.~Zhu$^{20}$, Y.~C.~Zhu$^{73,59}$, Z.~A.~Zhu$^{1,65}$, X.~Y.~Zhuang$^{44}$, J.~H.~Zou$^{1}$, J.~Zu$^{73,59}$
\\
\vspace{0.2cm}
(BESIII Collaboration)\\
\vspace{0.2cm} {\it
$^{1}$ Institute of High Energy Physics, Beijing 100049, People's Republic of China\\
$^{2}$ Beihang University, Beijing 100191, People's Republic of China\\
$^{3}$ Bochum  Ruhr-University, D-44780 Bochum, Germany\\
$^{4}$ Budker Institute of Nuclear Physics SB RAS (BINP), Novosibirsk 630090, Russia\\
$^{5}$ Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, USA\\
$^{6}$ Central China Normal University, Wuhan 430079, People's Republic of China\\
$^{7}$ Central South University, Changsha 410083, People's Republic of China\\
$^{8}$ China Center of Advanced Science and Technology, Beijing 100190, People's Republic of China\\
$^{9}$ China University of Geosciences, Wuhan 430074, People's Republic of China\\
$^{10}$ Chung-Ang University, Seoul, 06974, Republic of Korea\\
$^{11}$ COMSATS University Islamabad, Lahore Campus, Defence Road, Off Raiwind Road, 54000 Lahore, Pakistan\\
$^{12}$ Fudan University, Shanghai 200433, People's Republic of China\\
$^{13}$ GSI Helmholtzcentre for Heavy Ion Research GmbH, D-64291 Darmstadt, Germany\\
$^{14}$ Guangxi Normal University, Guilin 541004, People's Republic of China\\
$^{15}$ Guangxi University, Nanning 530004, People's Republic of China\\
$^{16}$ Guangxi University of Science and Technology, Liuzhou 545006, People's Republic of China\\
$^{17}$ Hangzhou Normal University, Hangzhou 310036, People's Republic of China\\
$^{18}$ Hebei University, Baoding 071002, People's Republic of China\\
$^{19}$ Helmholtz Institute Mainz, Staudinger Weg 18, D-55099 Mainz, Germany\\
$^{20}$ Henan Normal University, Xinxiang 453007, People's Republic of China\\
$^{21}$ Henan University, Kaifeng 475004, People's Republic of China\\
$^{22}$ Henan University of Science and Technology, Luoyang 471003, People's Republic of China\\
$^{23}$ Henan University of Technology, Zhengzhou 450001, People's Republic of China\\
$^{24}$ Huangshan College, Huangshan  245000, People's Republic of China\\
$^{25}$ Hunan Normal University, Changsha 410081, People's Republic of China\\
$^{26}$ Hunan University, Changsha 410082, People's Republic of China\\
$^{27}$ Indian Institute of Technology Madras, Chennai 600036, India\\
$^{28}$ Indiana University, Bloomington, Indiana 47405, USA\\
$^{29}$ INFN Laboratori Nazionali di Frascati , (A)INFN Laboratori Nazionali di Frascati, I-00044, Frascati, Italy; (B)INFN Sezione di  Perugia, I-06100, Perugia, Italy; (C)University of Perugia, I-06100, Perugia, Italy\\
$^{30}$ INFN Sezione di Ferrara, (A)INFN Sezione di Ferrara, I-44122, Ferrara, Italy; (B)University of Ferrara,  I-44122, Ferrara, Italy\\
$^{31}$ Inner Mongolia University, Hohhot 010021, People's Republic of China\\
$^{32}$ Institute of Modern Physics, Lanzhou 730000, People's Republic of China\\
$^{33}$ Institute of Physics and Technology, Mongolian Academy of Sciences, Peace Avenue 54B, Ulaanbaatar 13330, Mongolia\\
$^{34}$ Instituto de Alta Investigaci\'on, Universidad de Tarapac\'a, Casilla 7D, Arica 1000000, Chile\\
$^{35}$ Jilin University, Changchun 130012, People's Republic of China\\
$^{36}$ Johannes Gutenberg University of Mainz, Johann-Joachim-Becher-Weg 45, D-55099 Mainz, Germany\\
$^{37}$ Joint Institute for Nuclear Research, 141980 Dubna, Moscow region, Russia\\
$^{38}$ Justus-Liebig-Universitaet Giessen, II. Physikalisches Institut, Heinrich-Buff-Ring 16, D-35392 Giessen, Germany\\
$^{39}$ Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{40}$ Liaoning Normal University, Dalian 116029, People's Republic of China\\
$^{41}$ Liaoning University, Shenyang 110036, People's Republic of China\\
$^{42}$ Nanjing Normal University, Nanjing 210023, People's Republic of China\\
$^{43}$ Nanjing University, Nanjing 210093, People's Republic of China\\
$^{44}$ Nankai University, Tianjin 300071, People's Republic of China\\
$^{45}$ National Centre for Nuclear Research, Warsaw 02-093, Poland\\
$^{46}$ North China Electric Power University, Beijing 102206, People's Republic of China\\
$^{47}$ Peking University, Beijing 100871, People's Republic of China\\
$^{48}$ Qufu Normal University, Qufu 273165, People's Republic of China\\
$^{49}$ Renmin University of China, Beijing 100872, People's Republic of China\\
$^{50}$ Shandong Normal University, Jinan 250014, People's Republic of China\\
$^{51}$ Shandong University, Jinan 250100, People's Republic of China\\
$^{52}$ Shanghai Jiao Tong University, Shanghai 200240,  People's Republic of China\\
$^{53}$ Shanxi Normal University, Linfen 041004, People's Republic of China\\
$^{54}$ Shanxi University, Taiyuan 030006, People's Republic of China\\
$^{55}$ Sichuan University, Chengdu 610064, People's Republic of China\\
$^{56}$ Soochow University, Suzhou 215006, People's Republic of China\\
$^{57}$ South China Normal University, Guangzhou 510006, People's Republic of China\\
$^{58}$ Southeast University, Nanjing 211100, People's Republic of China\\
$^{59}$ State Key Laboratory of Particle Detection and Electronics, Beijing 100049, Hefei 230026, People's Republic of China\\
$^{60}$ Sun Yat-Sen University, Guangzhou 510275, People's Republic of China\\
$^{61}$ Suranaree University of Technology, University Avenue 111, Nakhon Ratchasima 30000, Thailand\\
$^{62}$ Tsinghua University, Beijing 100084, People's Republic of China\\
$^{63}$ Turkish Accelerator Center Particle Factory Group, (A)Istinye University, 34010, Istanbul, Turkey; (B)Near East University, Nicosia, North Cyprus, 99138, Mersin 10, Turkey\\
$^{64}$ University of Bristol, H H Wills Physics Laboratory, Tyndall Avenue, Bristol, BS8 1TL, UK\\
$^{65}$ University of Chinese Academy of Sciences, Beijing 100049, People's Republic of China\\
$^{66}$ University of Groningen, NL-9747 AA Groningen, The Netherlands\\
$^{67}$ University of Hawaii, Honolulu, Hawaii 96822, USA\\
$^{68}$ University of Jinan, Jinan 250022, People's Republic of China\\
$^{69}$ University of Manchester, Oxford Road, Manchester, M13 9PL, United Kingdom\\
$^{70}$ University of Muenster, Wilhelm-Klemm-Strasse 9, 48149 Muenster, Germany\\
$^{71}$ University of Oxford, Keble Road, Oxford OX13RH, United Kingdom\\
$^{72}$ University of Science and Technology Liaoning, Anshan 114051, People's Republic of China\\
$^{73}$ University of Science and Technology of China, Hefei 230026, People's Republic of China\\
$^{74}$ University of South China, Hengyang 421001, People's Republic of China\\
$^{75}$ University of the Punjab, Lahore-54590, Pakistan\\
$^{76}$ University of Turin and INFN, (A)University of Turin, I-10125, Turin, Italy; (B)University of Eastern Piedmont, I-15121, Alessandria, Italy; (C)INFN, I-10125, Turin, Italy\\
$^{77}$ Uppsala University, Box 516, SE-75120 Uppsala, Sweden\\
$^{78}$ Wuhan University, Wuhan 430072, People's Republic of China\\
$^{79}$ Yantai University, Yantai 264005, People's Republic of China\\
$^{80}$ Yunnan University, Kunming 650500, People's Republic of China\\
$^{81}$ Zhejiang University, Hangzhou 310027, People's Republic of China\\
$^{82}$ Zhengzhou University, Zhengzhou 450001, People's Republic of China\\

\vspace{0.2cm}
$^{b}$ Deceased\\
$^{c}$ Also at the Moscow Institute of Physics and Technology, Moscow 141700, Russia\\
$^{d}$ Also at the Novosibirsk State University, Novosibirsk, 630090, Russia\\
$^{e}$ Also at the NRC "Kurchatov Institute", PNPI, 188300, Gatchina, Russia\\
$^{f}$ Also at Goethe University Frankfurt, 60323 Frankfurt am Main, Germany\\
$^{g}$ Also at Key Laboratory for Particle Physics, Astrophysics and Cosmology, Ministry of Education; Shanghai Key Laboratory for Particle Physics and Cosmology; Institute of Nuclear and Particle Physics, Shanghai 200240, People's Republic of China\\
$^{h}$ Also at Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, People's Republic of China\\
$^{i}$ Also at State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing 100871, People's Republic of China\\
$^{j}$ Also at School of Physics and Electronics, Hunan University, Changsha 410082, China\\
$^{k}$ Also at Guangdong Provincial Key Laboratory of Nuclear Science, Institute of Quantum Matter, South China Normal University, Guangzhou 510006, China\\
$^{l}$ Also at MOE Frontiers Science Center for Rare Isotopes, Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{m}$ Also at Lanzhou Center for Theoretical Physics, Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{n}$ Also at the Department of Mathematical Sciences, IBA, Karachi 75270, Pakistan\\
$^{o}$ Also at Ecole Polytechnique Federale de Lausanne (EPFL), CH-1015 Lausanne, Switzerland\\
$^{p}$ Also at Helmholtz Institute Mainz, Staudinger Weg 18, D-55099 Mainz, Germany\\
$^{q}$ Also at Hangzhou Institute for Advanced Study, University of Chinese Academy of Sciences, Hangzhou 310024, China\\

}
%% ends here %%

